Can 100 Machines Agree?

Agreement protocols have been typically deployed at small scale, e.g., using three to five machines. This is because these protocols seem to suffer from a sharp performance decay. More specifically, as the size of a deployment---i.e., degree of replication---increases, the protocol performance greatly decreases. There is not much experimental evidence for this decay in practice, however, notably for larger system sizes, e.g., beyond a handful of machines. In this paper we execute agreement protocols on up to 100 machines and observe on their performance decay. We consider well-known agreement protocols part of mature systems, such as Apache ZooKeeper, etcd, and BFT-Smart, as well as a chain and a novel ring-based agreement protocol which we implement ourselves. We provide empirical evidence that current agreement protocols execute gracefully on 100 machines. We observe that throughput decay is initially sharp (consistent with previous observations); but intriguingly---as each system grows beyond a few tens of replicas---the decay dampens. For chain- and ring-based replication, this decay is slower than for the other systems. The positive takeaway from our evaluation is that mature agreement protocol implementations can sustain out-of-the-box 300 to 500 requests per second when executing on 100 replicas on a wide-area public cloud platform. Chain- and ring-based replication can reach between 4K and 11K (up to 20x improvements) depending on the fault assumptions.

==> sections/evaluation-cluster.tex <==
%!TEX root = ../tr.tex

\subsection{OpenStack Evaluation Resuts}
\label{sec:evaluation-cluster}

We also run additional experiments on an OpenStack cluster~\cite{openstack}.
The machine in this cluster have average inter-node latencies of $0.6$ms.
Physical nodes are interconnected with $10$Gbps networking, with \emph{netperf} and \emph{iperf} consistently reporting at least 8.5 Gbps effective throughput among VMs.
The VMs we use have the same characteristics as the ones in SoftLayer ($2$ virtual CPU cores and $4$GB RAM).

For these experiments, all system parameters, our methodology, and experimental setup are the same as the ones we use in the experiments on SoftLayer.
The OpenStack platform allows us to verify whether our earlier findings on the scalability of SMR systems also apply in a cluster environment.
In these experiments we only study the behavior of etcd, ZooKeeper, BFT-Smart, and \chainr.
In future work, we plan to also include our \name system, and to consider the impact of CPU and memory configurations.
Despite these results being more noisy that our experiments on the SoftLayer testbed, they serve to support our main claim that SMR can scale past a few replicas.
This cluster testbed is a virtualized environment shared with other researchers, so the resources available for our experiments are more limited and they fluctuate in time, in the sense that we cannot always get access to the same amount of virtual instances.\footnote{In the SoftLayer public cloud, we did not have this problem. The SoftLayer geo-replicated testbed has an on-demand model, and can scale elastically.}
We experiment with up to roughly $43$ replicas.

\textbf{Throughput.}
To help in the comparison between the two platforms, we plot the results for OpenStack side by side with the results we obtain in SoftLayer.
The results are in~\Cref{fig:zk-zc2,fig:etcd-zc2,fig:bfts-zc2,fig:chainr-zc2}, for each of the four systems we consider.
Before we discuss the results, we remark that in these experiments we use an unoptimized version of the \chainr system, where batching is not used.
Consequently, the throughput this system can sustain is lower, as~\Cref{fig:chainr-zc2} shows; the results in this figure for the SoftLayer testbed are also obtained by using the same unoptimized version of \chainr.
Nevertheless, the same trend is evident: the system maintains its throughput very well despite increasing system size.

We observe that, overall, the results for the two platforms are almost overlapping.
A notable difference in throughput appears for ZooKeeper, as revealed in~\Cref{fig:zk-zc2}.
First, the throughput is higher on the OpenStack cluster, but also more noisy than in the SoftLayer testbed.
We recall that each data point in the figure is the average of three executions.
So we observe that these results are consistent within a given configuration, e.g., all three executions with $N=7$ consistently yield a peak throughput of roughly $5.7k$ tps, hence the standard deviation (illustrated through whiskers) is very small.
But inconsistencies appear when we switch to a different configuration, i.e., when we include additional replicas, suggesting that throughput differences are simply a consequence of the additional replicas.
Notice, however, that throughput also \emph{increases} across subsequent configurations, e.g., peak throughput is higher with $N=11$ than with $N=7$; this can happen if the four additional replicas (in the $11$-replica system) have less interference and replace any slow replicas (that are part of the $7$-replica configuration).

On the OpenStack platform we used smaller system sizes (up to $43$), so it is not so obvious to observe how the throughput degradation tapers off as each system size increases.
But this trend does start manifesting to some degree at least starting with $N=23$.

\textbf{Latency.}
In terms of latency, we show the results for all four systems in~\Cref{fig:latencies-zc2}.
We note on the very low latencies achieved by \chainr , since now we no longer employ any form of batching, and latencies are sub-millisecond.
Otherwise, the results are very similar to our findings on the wide-area network of the SoftLayer testbed (\Cref{fig:latencies-sl}).


\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{../draft/figures/zk-zc2-numbers}}
\caption{Scalability experiments for Apache ZooKeeper on the OpenStack testbed.}
\label{fig:zk-zc2}
\end{figure}

\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{../draft/figures/etcd-zc2-numbers}}
\caption{Scalability experiments for etcd on the OpenStack testbed.}
\label{fig:etcd-zc2}
\end{figure}


\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{../draft/figures/bfts-zc2-numbers}}
\caption{Scalability experiments for BFT-Smart on the OpenStack testbed.}
\label{fig:bfts-zc2}
\end{figure}

\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{../draft/figures/chainr-zc2-numbers}}
\caption{Scalability experiments for the \chainr system on the OpenStack testbed. In this evaluation, we did not use batching, hence the results are different from those we present in~\Cref{fig:scalability-1}. The main difference is that, in the absence of batching, this system achieves lower throughput. Experiments with the same configuration on the SoftLayer testbed revealed, as expected, similar findings.}
\label{fig:chainr-zc2}
\end{figure}

\begin{figure*}[t]
\centerline{\includegraphics[width=.8\textwidth]{../draft/figures/latencies-zc2}}
\caption{Latency results for all four systems we study on the OpenStack platform.}
\label{fig:latencies-zc2}
\end{figure*}

